The Limitations of Large Width in Neural Networks: A Deep Gaussian Process Perspective

Large width limits have been a recent focus of deep learning research: modulo computational practicalities, do wider networks outperform narrower ones? Answering this question has been challenging, as conventional networks gain representational power with width, potentially masking any negative effects. Our analysis in this paper decouples capacity and width via the generalization of neural networks to Deep Gaussian Processes (Deep GP), a class of nonparametric hierarchical models that subsume neural nets. In doing so, we aim to understand how width affects (standard) neural networks once they have sufficient capacity for a given modeling task. Our theoretical and empirical results on Deep GP suggest that large width can be detrimental to hierarchical models. Surprisingly, we prove that even nonparametric Deep GP converge to Gaussian processes, effectively becoming shallower without any increase in representational power. The posterior, which corresponds to a mixture of data-adaptable basis functions, becomes less data-dependent with width. Our tail analysis demonstrates that width and depth have opposite effects: depth accentuates a model's non-Gaussianity, while width makes models increasingly Gaussian. We find there is a "sweet spot" that maximizes test performance before the limiting GP behavior prevents adaptability, occurring at width = 1 or width = 2 for nonparametric Deep GP. These results make strong predictions about the same phenomenon in conventional neural networks trained with L2 regularization (analogous to a Gaussian prior on parameters): we show that such neural networks may need up to 500 - 1000 hidden units for sufficient capacity - depending on the dataset - but further width degrades performance.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors\ldots
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \cref{sec:broader_impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Assumptions are listed in the theorem/lemma statements, as well as in \cref{sec:assumptions}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See \cref{sec:proof_dgp_gp,sec:proof_tails,sec:dgp_second_moments}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code is in supplementary.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:experimental_details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{%
      Our results for optimized networks are run 3-5 times, and indicate as such in the results figures.
      Due to compute resource constraints we only have one HMC run for each experiment in \cref{sec:experiments_bayesian}.
    }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \cref{sec:experimental_details}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{
      In \cref{sec:experiments_bayesian,sec:experiments_optimized} we supply citations for all datasets.
      In \cref{sec:experimental_details} we supply citations for all software packages.
    }
  \item Did you mention the license of the assets?
    \answerNo{
      To the best of our knowledge, none of the datasets we use have licenses.
      We mention that all software packages we use are open source.
    }
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{
      We use commonly-available public datasets that,
      to the best of our knowledge, do not pose any privacy or content concerns.
    }
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> scratch.tex <==
\newpage
\section*{Old work below}


\paragraph{Additional observations for 2-layer additive Deep GP.}
The additive and generative Deep GP represent two different classes of behavior in their infinite-width limit.
In the additive case, the first two moments of the prior remain constant with $H$.
However, the distribution of $h_\text{add}(\cdot)$ itself changes as $H$ increases: from a Deep GP to a (shallow) GP.
The general Deep GP exhibits different behavior.
Its second moment changes with $H$ while its tails also become more Gaussian.


\paragraph{Additional observations for general Deep GP.}
In the general case, how width affects the second moment depends on the choice of $k_g(\cdot, \cdot)$.
For example, if $k_g(\cdot, \cdot)$ is a (non-additive) RBF kernel, width results in faster decaying covariance functions.
To decouple covariance and width, we can make use of the following construction:
%
\begin{observation}
  Let $g(\bfn(\cdot))$ be a 2-layer zero-mean Deep GP of width-$H$.
  There exists a width-$1$ Deep GP $g'(f'(\cdot))$ with an equivalent second moment.
\end{observation}
\begin{proof}
  Let $k_g(\cdot, \cdot): \reals^{H \times H} \to \reals$ be the covariance function of $g(\cdot)$.
  The covariance of $g(\bfn(\cdot))$ is given by:
  %
  \begin{align*}
    \Ev{g(\bfn(\bx)) g(\bfn(\bx'))}
    &= \int k_g(\bfn(\bx), \bfn(\bx')) \: p(\bfn(\bx)) \: p(\bfn(\bx')) \intd \bfn(\bx) \intd \bfn(\bx').
    \\
    &= \int k_g(\bfn(\bx), \bfn(\bx')) \: \prod_{i=1}^H \left[ p(f_i(\bx)) \: p(f_i(\bx')) \right] \intd f_1(\bx) \ldots \intd f_H(\bx').
  \end{align*}
  %
  Let $k_g'(\cdot, \cdot)$ be defined as:
  %
  \begin{align*}
    k_g'(f(\bx), f(\bx'))
    &= \int k_g(\bfn(\bx), \bfn(\bx')) \: \prod_{i=1}^{H-1} \left[ p(f_i(\bx)) \: p(f_i(\bx')) \right] \intd f_1(\bx) \ldots \intd f_{H-1}(\bx').
  \end{align*}
  %
  In other words, $k_g'(f(\bx), f(\bx))$ is the covariance of $g(\bfn(\cdot))$ without $f_H(\bx), f_H(\bx')$ marginalized out.
  A simple manipulation of kernel construction rules will show that $k_g'(\cdot, \cdot)$ is a valid kernel.
  If we set $k_g'$ as the covariance function of $g'$, then $g'(f'(\cdot))$ will have the same second moment as $g(\bfn(\cdot))$.
\end{proof}
%
It is worth noting that the tails of this width-$1$ construction will be more Gaussian than that of $g(\bfn(\bx))$.
(This can be proved with a simple application of Jensen's inequality.)

\paragraph{Additional observations for stationary Deep GP.}
\begin{observation}
  Let $h(\cdot) = g(\bfn(\cdot))$ be a 2-layer zero-mean Deep GP.
  If $k_g$ is a stationary kernel---or more generally, if $k_g(\bz, \bz') = o^2$ for all $\bz \in \reals^H$---then the marginal distributions $p\left( h(\bx) \right)$ are Gaussian.
\end{observation}
%
\begin{proof}
  The Gaussian distribution satisfies Carleman's condition, and therefore is uniquely determined by its moments.
  Consequentially, our proof strategy is showing that the moments of $h(\bx)$ match that of a Gaussian.
  For any $R \in \mathcal{N}$, we have that:
  %
  \begin{align*}
    \Evover{h(\cdot)}{ h(\bx)^R }
    &=
    \Evover{\bfn(\cdot)}{ \Evover{g(\cdot) \mid \bfn(\cdot) }{ g( \bfn(\bx) )^R } }.
  \end{align*}
  %
  Since $g(\cdot) \mid \bfn(\cdot)$ is a zero-Gaussian process, the inner expectation is the $R^\text{th}$ moment of a zero-mean Gaussian.
  For odd $R$, we thus have $\Evover{h(\cdot)}{ h(\bx)^R } = \Evover{\bfn(\cdot)}{0} = 0$.
  For even $R$, we have
  $$
    \Evover{h(\cdot)}{h(\bx)^R } = \Evover{\bfn(\cdot)}{ (R-1)!! \: k( \bfn(\bx), \bfn(\bx))^{R / 2} }
    = \Evover{\bfn(\cdot)}{ (R-1)!! \: o^R } = (R-1)!! \: o^R.
  $$
  Thus the moments of $h(\bx)$ match that of a Gaussian with zero mean and variance $o^2$.
\end{proof}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

